Fundamental Limits of Low-Rank Matrix Estimation with Diverging Aspect Ratios

We consider the problem of estimating the factors of a low-rank $n \times d$ matrix, when this is corrupted by additive Gaussian noise. A special example of our setting corresponds to clustering mixtures of Gaussians with equal (known) covariances. Simple spectral methods do not take into account the distribution of the entries of these factors and are therefore often suboptimal. Here, we characterize the asymptotics of the minimum estimation error under the assumption that the distribution of the entries is known to the statistician. Our results apply to the high-dimensional regime $n, d \to \infty$ and $d / n \to \infty$ (or $d / n \to 0$) and generalize earlier work that focused on the proportional asymptotics $n, d \to \infty$, $d / n \to \delta \in (0, \infty)$. We outline an interesting signal strength regime in which $d / n \to \infty$ and partial recovery is possible for the left singular vectors while impossible for the right singular vectors. We illustrate the general theory by deriving consequences for Gaussian mixture clustering and carrying out a numerical study on genomics data.

==> background.tex <==
\section{Background and preliminaries}

We collect in this section some background knowledge and preliminaries for readers' convenience. We first give definitions of the GOE matrix and the pseudo-Lipschitz functions. 

\begin{definition}[Gaussian orthogonal ensemble]\label{def:GOE} For $n \in \NN_+$ and an $n$ by $n$ random matrix $\bW$, we say $\bW \overset{d}{=} \GOE(n)$ if and only if $\bW = \bW^{\top}$, $(W_{ij})_{1 \leq i < j \leq n} \iidsim \normal(0,1)$ and $(W_{ii})_{1 \leq i \leq n} \iidsim \normal(0,2)$.   
 	
 \end{definition}
 
 
\begin{definition}[pseudo-Lipschitz function]
	We say that a function $\phi: \mathbb{R}^m \rightarrow \mathbb{R}$ is pseudo-Lipschitz of order $k$ with $k \geq 1$, if there exists a constant $L > 0$ such that, for all $\vec x,\vec y \in \mathbb{R}^m$, 
	\begin{align*}
		|\phi(\vec{x}) - \phi(\vec y)| \leq L(1 + \|\vec x\|^{k - 1} + \|\vec y\|^{k - 1})\|\vec x - \vec y\|.
	\end{align*}
	In this case, we say $\phi \in \mathrm{PL}(k)$. 
\end{definition}
\begin{remark}
	If $f(x), g(x)$ are Lipschitz continuous functions, then $f(x)g(x)$ is pseudo-Lipschitz of order 2.  
\end{remark}
\begin{comment}
	\begin{definition}[Wasserstein distance]
	For $k \in \NN_+$, let $\mu_1, \mu_2$ be two probability distributions over $\RR^r$, recall that the Wasserstein distance between $\mu_1$ and $\mu_2$ is defined as
\begin{align}
	W_2(\mu_1, \mu_2) = \left( \inf_{\gamma \in \Gamma(\mu_1, \mu_2)} \int_{\RR^k \times \RR^k} \|x - y\|^2 \dd \gamma(x, y) \right)^{1/2},
\end{align}
where $\Gamma(\mu_1, \mu_2)$ denote the collection of all probability distributions over $\RR^k \times \RR^k$ with marginals $\mu_1$ and $\mu_2$ on the first and last $k$ coordinates, respectively.
\end{definition}

\end{comment}




\subsection{Properties of the symmetric spiked model}

We first give a definition of the symmetric spiked model. Given signal-to-noise ratio $s > 0$, under this model we observe a symmetric matrix $\bY \in \RR^{n \times n}$ satisfying 
%
\begin{align}\label{model:spike}
	\bY = \frac{\sqrt{s}}{n}\bLambda\bLambda^{\top} + \bW,
\end{align}
%
where $\bW \overset{d}{=} \frac{1}{\sqrt{n}} \GOE(n)$ and $\Lambda_i \iidsim \mu_{\Lambda}$, independent of each other. 
For readers' convenience, we collect in this section some useful properties of the symmetric spiked model. We refer the interested readers to \cite{lelarge2019fundamental} for more details. As preliminary knowledge, we define
%
\begin{align}
	& \bQ^{\ast}(s) := \sup_{\bQ \in S_r^+} \cF(s, \bQ), \label{eq:Qstar}\\
	& \cF(s, \bQ) := -\frac{s}{4}\|\bQ\|_F^2 + \E_{Z \sim \normal(0, \id_r), \Lambda \sim \mu_{\Lambda}}\log \left( \int \exp(\sqrt{s}Z^{\top} \bQ^{1/2}\lambda + s\lambda^{\top} \bQ\Lambda - \frac{s}{2}\lambda^{\top} \bQ\lambda)\dd\mu_{\Lambda}(\lambda) \right).\label{eq:FsQ}
\end{align}
%
In the above expression the expectation is taken over $\Lambda \sim \mu_{\Lambda}, Z \sim \normal(0, \id_r)$ with $Z \perp \Lambda$.
%
\begin{proposition}[\cite{lelarge2019fundamental}, Proposition 44, Corollary 45]\label{prop:symmetric-spike}
	For all but countably many $s \geq 0$, all the maximizers of \cref{eq:Qstar} have the same Frobenius norm, and
	\begin{align*}
	\lim_{n\rightarrow \infty}\frac{1}{n^2} \inf_{\hat{\bM}(\bY)}\E\left[ \| \bLambda\bLambda^{\top} - \hat{\bM}(\bY)   \|_F^2 \right] = \|\E_{\Lambda \sim \mu_{\Lambda}}[\Lambda \Lambda^{\top}]\|_F^2 - \|\bQ^{\ast}(s)\|_F^2.
\end{align*}

\end{proposition}


  

\subsection{Approximate message passing (AMP)}

In this section we summarize the main properties of the AMP algorithm, focusing on Bayes AMP with spectral initialization for the problem of symmetric rank-one matrix estimation \eqref{model:spike} \cite{montanari2017estimation}. We let $\bvarphi \in \RR^n$ be the top eigenvector of $\bY$. The Bayes AMP algorithm with spectral initialization proceeds iteratively as follows:
%
\begin{align*}
	& \vlambda^0 = \sqrt{n s(s - 1)} \bvarphi, \\
	& \vlambda^{t + 1} = \bY f_t(\vlambda^t) - b_t f_{t - 1}(\vlambda^{t - 1}), \qquad b_t = \frac{1}{n}\sum_{i = 1}^n f_t'(\lambda_i^t).
\end{align*}
%
Let $\Lambda \sim \mu_{\Lambda}$ and $G \sim \normal(0,1)$. Without loss of generality we assume $\E[\Lambda^2] = 1$. We define the minimum mean square error upon observing $\sqrt{\gamma} \Lambda + G$ as
%
\begin{align*}
	\mathsf{mmse}(\gamma) = \E[(\Lambda - \E[\Lambda \mid \sqrt{\gamma} \Lambda + G])^2].
\end{align*}
%
With these notations, we can introduce the state evolution recursion 
%
\begin{align*}
	& \gamma_0 = s - 1, \\
	& \gamma_{t + 1} = s(1 - \mathsf{mmse}(\gamma_t)).
\end{align*}
%
Maximizing the signal-to-noise ratio at every step, we see that the optimal non-linearity $f_t$ takes the form of conditional expectation:
%
\begin{align*}
	f_t(y) = \sqrt{s} \E[\Lambda \mid \gamma_t \Lambda + \sqrt{\gamma_t} G = y].
\end{align*}
%
The following theorem characterizes the asymptotic behavior of Bayes AMP under the above choice of non-linearity.
\begin{theorem}
	Assume $f_t$ is Lipschitz continuous for any $\gamma \in (0, s]$, then for any $\psi: \RR^2 \to \RR$ such that $\psi \in \mathrm{PL}(2)$, almost surely we have
	\begin{align*}
		\lim_{n \to \infty} \frac{1}{n} \sum_{i = 1}^n \psi(\Lambda_i, \lambda_i^t) = \E[\psi(\Lambda, \gamma_t \Lambda + \gamma_t^{1/2} G)].
	\end{align*}
\end{theorem}
%
According to \cite[Corollary 2.3]{montanari2017estimation}, we see that Bayes AMP asymptotically achieves Bayes optimal error if and only if the following condition holds:
%
\begin{condition}\label{condition:stationary}
	For $Y = \sqrt{\gamma} \Lambda + G$, we define $\mathsf{I}(\gamma) = \E \log \frac{\dd p_{Y \mid \Lambda}}{\dd p_Y}(Y, \Lambda)$ as the mutual information between $Y$ and $\Lambda$. Let 
	%
	\begin{align*}
		\Psi(\gamma, s) = \frac{s}{4} + \frac{\gamma^2}{4\sqrt{s}} - \frac{\gamma}{2} + \mathsf{I}(\gamma).
	\end{align*}
	%
	This condition requires that the global maximum of $\gamma \mapsto \Psi(\gamma, s)$ over $(0, \infty)$ is also the first stationary point of the same function. 
\end{condition}

% Broadly speaking, past works characterizing computational or information theoretic phase transitions fall into two categories. For works in the first category, upper and lower bounds on the phase transition thresholds are derived, which typically follows with finite-sample guarantees. Usually there is a constant or logarithmic multiplicative gap between the obtained bounds. We refer to \cite{giraud2018partial,ndaoud2018sharp,berthet2013computational,cai2017computational} for exemplar works of this type.
 
%On the other hand, works in the second category delineate exact phase transition thresholds. Their derivations usually rely on more stringent modeling assumptions, and their results only hold asymptotically. Moreover, these works are typically based on tools from statistical mechanics and random matrix theory, thus almost always requiring constant aspect ratio (i.e., $n / d \rightarrow \alpha \in (0, \infty)$). Here we list a few representatives in this category. Note that the following results are all obtained under the condition $n / d \rightarrow \alpha \in (0, \infty)$. 

%\vspace{0.2cm}
%\noindent
%\textbf{Phase transition of the top singular values} 

%\noindent
%The phase transition phenomenon for the top singular values was first discovered in the physics literature \cite{edwards1976eigenvalue}, and later rigorously proved in the following works \cite{baik2005phase,baik2006eigenvalues,benaych2011eigenvalues, benaych2012singular}. Here we state the more recent results from \cite{benaych2012singular}. Under model \eqref{model:general}, we let $\bQ_{\Lambda} = \Cov(\Lambda) \in \RR^{r \times r}$ and $\bQ_{\Theta} = \Cov(\Theta) \in \RR^{r \times r}$. We further assume $n / d \rightarrow \alpha \in (0, 1]$ and $s_n = n^{-1/2}$. We denote the $r$ singular values of $\bQ_{\Lambda}^{1/2} \bQ_{\Theta}^{1/2}$ by $\sigma_1 \geq  \cdots \geq \sigma_r \geq 0$. Here $\bQ_{\Lambda}^{1/2}$, $\bQ_{\Theta}^{1/2}$ are positive semi-definite matrices satisfying $\bQ_{\Lambda}^{1/2}\bQ_{\Lambda}^{1/2} = \bQ_{\Lambda}$ and $\bQ_{\Theta}^{1/2}\bQ_{\Theta}^{1/2} = \bQ_{\Theta}$, respectively. For any $i \in [r]$, we let $\sigma_i(\bA / \sqrt{d})$ be the $i$-th largest singular value of $\bA / \sqrt{d}$, then as $n,d \rightarrow \infty$, 
%\begin{align*}
%	\sigma_i(\bA / \sqrt{d}) \overset{a.s.}{\rightarrow} \left\{ \begin{array}{ll}
%		\sqrt{(\alpha + \sigma_i^2)(1 + \sigma_i^2)\sigma_i^{-2}} & \mbox{if $\sigma_i > \alpha^{1/4}$}, \\
%		1 + \sqrt{\alpha} & \mbox{otherwise}. 
%	\end{array} \right.
%\end{align*}

%\vspace{0.2cm}
%\noindent
%\textbf{Limiting expression of the Bayesian MMSE} 




%Unfortunately, all the works cited here either fail to derive the exact limit of information-theoretic threshold, or fall short of addressing the non-fixed aspect ratio setting in which $d / n \rightarrow \infty$. In this paper, we aim to derive the exact expression for the limiting MMSE of $\bLambda$ and $\bTheta$, respectively, under the modeling assumption \eqref{model:general} and $d / n \rightarrow \infty$. As a natural corollary, we locate the exact information-theoretic threshold for estimation of $\bLambda$ and $\bTheta$. 

\subsection{Loss functions}\label{sec:loss-functions}
In this section we discuss various loss functions that will be employed in this paper. 
%
\subsubsection*{Vector mean squared error}
%
We first consider the standard vector mean squared error $L^v$. For $\bhLambda \in \RR^{n \times r}$ and $\hat\bTheta \in \RR^{d \times r}$ that are estimates of the low-rank signals $\bLambda$ and $\bTheta$ respectively, the vector mean squared errors of the estimation are defined as follows:
%
\begin{align*}
	L^v(\bLambda, \bhLambda) := \frac{1}{n}\|\bLambda - \bhLambda\|_F^2, \qquad \qquad L^v(\bTheta, \hat\bTheta) := \frac{1}{d}\|\bTheta - \hat\bTheta\|_F^2. 
\end{align*} 
%
In the above display $\|\cdot\|_F$ stands for the Frobenius norm. We comment that sometimes $L^v$ is not a reasonable loss function due to potential non-identifiability issue (i.e., $\bLambda \bTheta^{\top} = \bLambda \Omega\Omega^{-1}\bTheta^{\top}$ for $\Omega \in \mathcal{O}(r)$). Under the Bayesian setting considered here, the existence of non-identifiability issue crucially depends on whether the prior distributions  $(\mu_{\Lambda}, \mu_{\Theta})$ are strong enough to settle the underlying uncertainty. To see a negative example, we let $\mu_{\Lambda} = \Unif\{\be_1, \be_2, \cdots, \be_r\}$ and $\mu_{\Theta} = \normal(0, \id_r)$, where $\be_i \in \RR^r$ with the $i$-th coordinate being 1 and all the rest being 0. This is a model used for the purpose of Gaussian mixture clustering. Then we immediately see that under such modeling assumption, it is impossible to separate the columns of the low-rank signals, thus vector mean squared error is not appropriate here. 

 
Later in \cref{thm:strong-signal-lambda-consistent} we will provide sufficient but not necessary conditions on $(\mu_{\Lambda}, \mu_{\Theta})$, such that under these conditions the non-identifiability issue can be eliminated. 
 
 % As a consequence, we will only apply the classical $l_2$ loss when symmetry breaking conditions are satisfied. A precise characterization of the symmetry breaking condition turns out to be quite subtle, and we provide a rough depiction in Theorem \ref{thm:strong-signal-lambda-consistent}. 
 
 \subsubsection*{Matrix mean squared error}

As an alternative of the vector mean squared error, we consider the matrix mean squared error. In words, we switch the goal of estimation from $\bLambda$, $\bTheta$ to $\bLambda \bLambda^{\top}$ and $\bTheta \bTheta^{\top}$, thus circumvent the potential non-identifiability issue. More precisely, for $\hat{\bM}_1 \in \RR^{n \times n}$ and $\hat{\bM}_2 \in \RR^{d \times d}$ that are estimators of $\bLambda  \bLambda^{\top}$ and $\bTheta  \bTheta^{\top}$, respectively, we define the corresponding matrix mean squared errors as 
%
\begin{align*}
	L(\bLambda\bLambda^{\top}, \hat{\bM}_{1}) := \frac{1}{n^2}\big\| \bLambda\bLambda^{\top} - \hat{\bM}_1 \big\|_F^2, \qquad \qquad L(\bTheta \bTheta^{\top}, \hat{\bM}_{2}) := \frac{1}{d^2}\big\| \bTheta \bTheta^{\top} - \hat{\bM}_{2}\big\|_F^2.
\end{align*}
%
The matrix mean squared error will also be the loss function adopted in our main theorem. 

\subsubsection*{Overlap between clusters}

As we have mentioned, in later parts of the paper we will apply our theorems to the problem of Gaussian mixture clustering, for which the mean squared error losses are no longer appropriate as the clustering results are typically discrete. For this part only, we consider the \emph{overlap} between clustering outcomes. 


Assume that we observe $n$ data points, with each data point belonging to one of $r$ clusters. Given the observations, our goal is to recover the underlying cluster assignments. We denote the cluster assignments of the samples by $\{\Lambda_i \in \{\be_j\}_{j \in [r]}\}_{i \in [n]}$. Here, $\Lambda_i = \be_j$ means that the $i$-th sample belongs to the $j$-th cluster. For $\{\hat\Lambda_i \in \{\be_j\}_{j \in [r]}\}_{i \in [n]}$ being an estimate of the cluster assignment, we define the overlap between the truth and its estimate as 
%
\begin{align*}
	\Overlap_n := \max_{\pi \in \mathfrak{S}_r }\frac{1}{n}\sum\limits_{i = 1}^n \mathbbm{1}\{\Lambda_i = \pi \circ \hat\Lambda_i\},
\end{align*}
where $\mathfrak{S}_r$ is the group of permutations over $\{\be_j\}_{j \in [r]}$. The goal is to design estimator which maximizes the overlap, with the resulting loss function formulated as $1 - \Overlap_n$. 



==> background_v2.tex <==
\section{Preliminaries}
\label{sec:Preliminaries}

%\am{Please remove from this section (or move to appendices) everything that
%is not strictly needed to understand the main text.}

We collect in this section some preliminary knowledge for readers' convenience. 
%We first give definitions of the GOE matrix and the pseudo-Lipschitz functions. 

%\begin{definition}[Gaussian orthogonal ensemble]\label{def:GOE} For $n \in \NN_+$ and an $n$ by $n$ random matrix $\bW$, we say $\bW \overset{d}{=} \GOE(n)$ if and only if $\bW = \bW^{\top}$, $(W_{ij})_{1 \leq i < j \leq n} \iidsim \normal(0,1)$ and $(W_{ii})_{1 \leq i \leq n} \iidsim \normal(0,2)$.   
 	
% \end{definition}
 
 
%\begin{definition}[pseudo-Lipschitz function]
%	We say that a function $\phi: \mathbb{R}^m \rightarrow \mathbb{R}$ is pseudo-Lipschitz of order $k$ with $k \geq 1$, if there exists a constant $L > 0$ such that, for all $\vec x,\vec y \in \mathbb{R}^m$, 
%	\begin{align*}
%		|\phi(\vec{x}) - \phi(\vec y)| \leq L(1 + \|\vec x\|^{k - 1} + \|\vec y\|^{k - 1})\|\vec x - \vec y\|.
%	\end{align*}
%	In this case, we say $\phi \in \mathrm{PL}(k)$. 
%\end{definition}
%\begin{remark}
%	If $f(x), g(x)$ are Lipschitz continuous functions, then $f(x)g(x)$ is pseudo-Lipschitz of order 2.  
%\end{remark}
\begin{comment}
	\begin{definition}[Wasserstein distance]
	For $k \in \NN_+$, let $\mu_1, \mu_2$ be two probability distributions over $\RR^r$, recall that the Wasserstein distance between $\mu_1$ and $\mu_2$ is defined as
\begin{align}
	W_2(\mu_1, \mu_2) = \left( \inf_{\gamma \in \Gamma(\mu_1, \mu_2)} \int_{\RR^k \times \RR^k} \|x - y\|^2 \dd \gamma(x, y) \right)^{1/2},
\end{align}
where $\Gamma(\mu_1, \mu_2)$ denote the collection of all probability distributions over $\RR^k \times \RR^k$ with marginals $\mu_1$ and $\mu_2$ on the first and last $k$ coordinates, respectively.
\end{definition}

\end{comment}




\subsection{Properties of the symmetric spiked model}

We introduce here the symmetric spiked model for completeness. Several useful properties of the model that are related to our results are listed below. Suppose $s > 0$ is the signal-to-noise ratio of the model. Under this model we observe $\bY \in \RR^{n \times n}$ satisfying 
%
\begin{align}\label{model:spike}
	\bY = \frac{\sqrt{s}}{n}\bLambda\bLambda^{\top} + \bW,
\end{align}
%
where $\bW \overset{d}{=}  \GOE(n)$ and $\bLambda_i \iidsim \mu_{\Lambda}$, independent of each other. 
For $s > 0$ and $\bQ \in S_r^+$, we define the following free energy functionals
%For readers' convenience, we collect in this section some useful properties of the symmetric spiked model. We refer the interested readers to \cite{lelarge2019fundamental} for more details. As preliminary knowledge, we define
%
\begin{align}
	& \bQ^{\ast}(s) := \sup_{\bQ \in S_r^+} \cF(s, \bQ), \label{eq:Qstar}\\
	& \cF(s, \bQ) := -\frac{s}{4}\|\bQ\|_F^2 + \E\left\{\log \left( \int \exp(\sqrt{s}\bz^{\top} \bQ^{1/2}\vlambda + s\vlambda^{\top} \bQ\bLambdas - \frac{s}{2}\vlambda^{\top} \bQ\vlambda)\mu_{\Lambda}(\dd\vlambda) \right)\right\}.\label{eq:FsQ}
\end{align}
%
In the above expression, the expectation is taken over $\bLambdas \sim \mu_{\Lambda}$ and  $\bz \sim \normal(0, \id_r)$ that are independent of each other. These functionals are directly related to the Bayesian MMSE of model \eqref{model:spike}, as stated by the following proposition. 
%
\begin{proposition}[\cite{lelarge2019fundamental}, Proposition 43]\label{prop:symmetric-spike}
	For all but countably many $s \geq 0$
	\begin{align*}
	\lim_{n\rightarrow \infty}\frac{1}{n^2} \inf_{\hat{\bM}(\bY)}\E\left[ \| \bLambda\bLambda^{\top} - \hat{\bM}(\bY)   \|_F^2 \right] = \|\E_{\bLambdas \sim \mu_{\Lambda}}[\bLambdas \bLambdas^{\top}]\|_F^2 - \|\bQ^{\ast}(s)\|_F^2.
\end{align*}

\end{proposition}


  

%\subsection{Approximate message passing (AMP)}

%In this section we summarize the main properties of the AMP algorithm, focusing on Bayes AMP with spectral initialization for the problem of symmetric rank-one matrix estimation \eqref{model:spike} \cite{montanari2021estimation}. 

%Let $\bvarphi \in \RR^n$ be the top eigenvector of $\bY$. The Bayes AMP algorithm  for model \eqref{model:spike} proceeds iteratively as follows:
%
%\begin{align*}
%	& \vlambda^0 = \sqrt{n s(s - 1)} \bvarphi, \\
%	& \vlambda^{t + 1} = \bY f_t(\vlambda^t) - b_t f_{t - 1}(\vlambda^{t - 1}), \qquad b_t = \frac{1}{n}\sum_{i = 1}^n f_t'(\lambda_i^t).
%\end{align*}
%
%Let $\Lambda \sim \mu_{\Lambda}$ and $G \sim \normal(0,1)$. Without loss of generality we assume $\E[\Lambda^2] = 1$. We define the minimum mean square error upon observing $\sqrt{\gamma} \Lambda + G$ as
%
%\begin{align*}
%	\mathsf{mmse}(\gamma) = \E[(\Lambda - \E[\Lambda \mid \sqrt{\gamma} \Lambda + G])^2].
%\end{align*}
%
%With these notations, we can introduce the state evolution recursion 
%
%\begin{align*}
%	& \gamma_0 = s - 1, \\
%	& \gamma_{t + 1} = s(1 - \mathsf{mmse}(\gamma_t)).
%\end{align*}
%
%Maximizing the signal-to-noise ratio at every step, we see that the optimal non-linearity $f_t$ takes the form of conditional expectation:
%
%\begin{align*}
%	f_t(y) = \sqrt{s} \E[\Lambda \mid \gamma_t \Lambda + \sqrt{\gamma_t} G = y].
%\end{align*}
%
%The following theorem characterizes the asymptotic behavior of Bayes AMP under the above choice of non-linearity.
%\begin{theorem}
%	Assume $f_t$ is Lipschitz continuous for any $\gamma \in (0, s]$, then for any $\psi: \RR^2 \to \RR$ such that $\psi \in \mathrm{PL}(2)$, almost surely we have
%	\begin{align*}
%		\lim_{n \to \infty} \frac{1}{n} \sum_{i = 1}^n \psi(\Lambda_i, \lambda_i^t) = \E[\psi(\Lambda, \gamma_t \Lambda + \gamma_t^{1/2} G)].
%	\end{align*}
%\end{theorem}
%
%According to \cite[Corollary 2.3]{montanari2021estimation}, this algorithm asymptotically achieves Bayes optimality if and only if the following condition holds:
%
%\begin{condition}\label{condition:stationary}
%	For $Y = \sqrt{\gamma} \Lambda + G$, we define $\mathsf{I}(\gamma) = \E \log \frac{\dd p_{Y \mid \Lambda}}{\dd p_Y}(Y, \Lambda)$ as the mutual information between $Y$ and $\Lambda$. Let 
	%
%	\begin{align*}
%		\Psi(\gamma, s) = \frac{s}{4} + \frac{\gamma^2}{4\sqrt{s}} - \frac{\gamma}{2} + \mathsf{I}(\gamma).
%	\end{align*}
	%
%	This condition requires that the global maximum of $\gamma \mapsto \Psi(\gamma, s)$ over $(0, \infty)$ is also the first stationary point of the same function. 
%\end{condition}

%\yw{I keep the most basic statement of AMP, to explain condition \ref{condition:stationary}}

% Broadly speaking, past works characterizing computational or information theoretic phase transitions fall into two categories. For works in the first category, upper and lower bounds on the phase transition thresholds are derived, which typically follows with finite-sample guarantees. Usually there is a constant or logarithmic multiplicative gap between the obtained bounds. We refer to \cite{giraud2018partial,ndaoud2022sharp,berthet2013computational,cai2017computational} for exemplar works of this type.
 
%On the other hand, works in the second category delineate exact phase transition thresholds. Their derivations usually rely on more stringent modeling assumptions, and their results only hold asymptotically. Moreover, these works are typically based on tools from statistical mechanics and random matrix theory, thus almost always requiring constant aspect ratio (i.e., $n / d \rightarrow \alpha \in (0, \infty)$). Here we list a few representatives in this category. Note that the following results are all obtained under the condition $n / d \rightarrow \alpha \in (0, \infty)$. 

%\vspace{0.2cm}
%\noindent
%\textbf{Phase transition of the top singular values} 

%\noindent
%The phase transition phenomenon for the top singular values was first discovered in the physics literature \cite{edwards1976eigenvalue}, and later rigorously proved in the following works \cite{baik2005phase,baik2006eigenvalues,benaych2011eigenvalues, benaych2012singular}. Here we state the more recent results from \cite{benaych2012singular}. Under model \eqref{model:general}, we let $\bQ_{\Lambda} = \Cov(\Lambda) \in \RR^{r \times r}$ and $\bQ_{\Theta} = \Cov(\Theta) \in \RR^{r \times r}$. We further assume $n / d \rightarrow \alpha \in (0, 1]$ and $s_n = n^{-1/2}$. We denote the $r$ singular values of $\bQ_{\Lambda}^{1/2} \bQ_{\Theta}^{1/2}$ by $\sigma_1 \geq  \cdots \geq \sigma_r \geq 0$. Here $\bQ_{\Lambda}^{1/2}$, $\bQ_{\Theta}^{1/2}$ are positive semi-definite matrices satisfying $\bQ_{\Lambda}^{1/2}\bQ_{\Lambda}^{1/2} = \bQ_{\Lambda}$ and $\bQ_{\Theta}^{1/2}\bQ_{\Theta}^{1/2} = \bQ_{\Theta}$, respectively. For any $i \in [r]$, we let $\sigma_i(\bA / \sqrt{d})$ be the $i$-th largest singular value of $\bA / \sqrt{d}$, then as $n,d \rightarrow \infty$, 
%\begin{align*}
%	\sigma_i(\bA / \sqrt{d}) \overset{a.s.}{\rightarrow} \left\{ \begin{array}{ll}
%		\sqrt{(\alpha + \sigma_i^2)(1 + \sigma_i^2)\sigma_i^{-2}} & \mbox{if $\sigma_i > \alpha^{1/4}$}, \\
%		1 + \sqrt{\alpha} & \mbox{otherwise}. 
%	\end{array} \right.
%\end{align*}

%\vspace{0.2cm}
%\noindent
%\textbf{Limiting expression of the Bayesian MMSE} 




%Unfortunately, all the works cited here either fail to derive the exact limit of information-theoretic threshold, or fall short of addressing the non-fixed aspect ratio setting in which $d / n \rightarrow \infty$. In this paper, we aim to derive the exact expression for the limiting MMSE of $\bLambda$ and $\bTheta$, respectively, under the modeling assumption \eqref{model:general} and $d / n \rightarrow \infty$. As a natural corollary, we locate the exact information-theoretic threshold for estimation of $\bLambda$ and $\bTheta$. 

\subsection{Loss functions}\label{sec:loss-functions}
In this section we discuss various loss functions that will be employed in this paper. 
%
\subsubsection*{Vector mean square error}
%
For $\bhLambda \in \RR^{n \times r}$ and $\hat\bTheta \in \RR^{d \times r}$ that are estimates of the factors $\bLambda$ and $\bTheta$, respectively, we define their (normalized) vector mean square errors as
%
\begin{align*}
	L^v(\bLambda, \bhLambda) := \frac{1}{n}\|\bLambda - \bhLambda\|_F^2, \qquad \qquad L^v(\bTheta, \hat\bTheta) := \frac{1}{d}\|\bTheta - \hat\bTheta\|_F^2. 
\end{align*} 
%
We comment that $L^v$ might not be an appropriate loss function under model \eqref{model:general}, due to potential non-identifiability issues. Later in \cref{thm:strong-signal-lambda-consistent} we discuss conditions on $(\mu_{\Lambda}, \mu_{\Theta})$ which allow us to overcome such problem. 

%We comment that sometimes $L^v$ is not a reasonable loss function due to potential non-identifiability issue (i.e., $\bLambda \bTheta^{\top} = \bLambda \Omega\Omega^{-1}\bTheta^{\top}$ for $\Omega \in \mathcal{O}(r)$). Under the Bayesian setting considered here, the existence of non-identifiability issue crucially depends on whether the prior distributions  $(\mu_{\Lambda}, \mu_{\Theta})$ are strong enough to settle the underlying uncertainty. To see a negative example, we let $\mu_{\Lambda} = \Unif\{\be_1, \be_2, \cdots, \be_r\}$ and $\mu_{\Theta} = \normal(0, \id_r)$, where $\be_i \in \RR^r$ with the $i$-th coordinate being 1 and all the rest being 0. This is a model used for the purpose of Gaussian mixture clustering. Then we immediately see that under such modeling assumption, it is impossible to separate the columns of the low-rank signals, thus vector mean squared error is not appropriate here. 

 
%Later in \cref{thm:strong-signal-lambda-consistent} we will provide sufficient but not necessary conditions on $(\mu_{\Lambda}, \mu_{\Theta})$, such that under these conditions the non-identifiability issue can be eliminated. 
 
 % As a consequence, we will only apply the classical $l_2$ loss when symmetry breaking conditions are satisfied. A precise characterization of the symmetry breaking condition turns out to be quite subtle, and we provide a rough depiction in Theorem \ref{thm:strong-signal-lambda-consistent}. 
 
 \subsubsection*{Matrix mean square error}

As an alternative, we consider the matrix mean square error. For $\hat{\bM}_1 \in \RR^{n \times n}$ and $\hat{\bM}_2 \in \RR^{d \times d}$ that are estimates of matrices $\bLambda  \bLambda^{\top}$ and $\bTheta  \bTheta^{\top}$, respectively, we define 
%
\begin{align*}
	L(\bLambda\bLambda^{\top}, \hat{\bM}_{1}) := \frac{1}{n^2}\big\| \bLambda\bLambda^{\top} - \hat{\bM}_1 \big\|_F^2, \qquad \qquad L(\bTheta \bTheta^{\top}, \hat{\bM}_{2}) := \frac{1}{d^2}\big\| \bTheta \bTheta^{\top} - \hat{\bM}_{2}\big\|_F^2.
\end{align*}
%
The matrix mean square error is also the loss function adopted in our main theorems. 

%\subsubsection*{Overlap between clusters}

%Mean square error losses might not be  appropriate for clustering problems in which the labels are discrete. In this case, we consider the \emph{overlap} between the estimated labels and the truth. 

%Suppose we have $n$ samples each belonging to one of $r$ clusters. If the $i$-th sample belongs to the $j$-th cluster, then we set $\bLambda_i = \be_j$. Here, $\be_j$ is the $j$-th standard basis in $\RR^r$. For $\{\hat\bLambda_i \in \{\be_j\}_{j \in [r]}\}_{i \in [n]}$ being an estimate of the cluster assignments, we define its overlap with the truth as
%
%As we have mentioned, in later parts of the paper we will apply our theorems to the problem of Gaussian mixture clustering, for which the mean squared error losses are no longer appropriate as the clustering results are typically discrete. For this part only, we consider the \emph{overlap} between clustering outcomes. 
%Given the observations, our goal is to recover the underlying cluster assignments. We denote the cluster assignments of the samples by $\{\Lambda_i \in \{\be_j\}_{j \in [r]}\}_{i \in [n]}$. Here, $\Lambda_i = \be_j$ means that the $i$-th sample belongs to the $j$-th cluster. For $\{\hat\Lambda_i \in \{\be_j\}_{j \in [r]}\}_{i \in [n]}$ being an estimate of the cluster assignment, we define the overlap between the truth and its estimate as 
%
%\begin{align*}
%	\Overlap_n := \max_{\pi \in \mathfrak{S}_r }\frac{1}{n}\sum\limits_{i = 1}^n \mathbbm{1}\{\bLambda_i = \pi \circ \hat\bLambda_i\},
%\end{align*}
%where $\mathfrak{S}_r$ is the group of permutations over $\{\be_j\}_{j \in [r]}$. We want to design classifiers that maximize the overlap, thus $1 - \Overlap_n$ serves as a reasonable loss function.   



==> copied_stuff.tex <==

%We write the posterior distributions under model \eqref{model:symmetric} and \eqref{model:weak-signal} as 
%%
\begin{align*}
	& \P(\dd \vlambda \mid \bY) = \frac{e^{-H_s(\vlambda)} \tensorl}{\int e^{-H_s(\vlambda)} \tensorl }, \\
	& \P(\dd\vlambda, \dd \vtheta \mid \bA) = \frac{e^{-H(\vlambda, \vtheta)} \tensort\tensorl}{\int e^{-H(\vlambda, \vtheta)} \tensort\tensorl},
\end{align*} 
where $ \tensorl$ ($\tensort$) is the product distribution over $\RR^n$ ($\RR^d$) with each coordinate having marginal distribution $\mu_{\Lambda}$ ($\mu_{\Theta}$), and $H_s, H$ are the Hamiltonians for model \eqref{model:symmetric} and \eqref{model:weak-signal}, respectively
%
\begin{align}\label{eq:Hs-and-H}
\begin{split}
	& H_s(\vlambda ) := \, \frac{q_{\Theta}^2}{2n}\langle \bLambda, \vlambda \rangle^2 + \frac{q_{\Theta}}{2}\vlambda^\sT\bW \vlambda - \frac{q_{\Theta}^2}{4n}\|\vlambda\|^4, \\
	& H(\vlambda, \vtheta) := \frac{1}{\sqrt{nd}}\langle \bLambda, \vlambda \rangle \langle \bTheta, \vtheta \rangle + \frac{1}{\sqrt[4]{nd}}  \vlambda^{\top}\bZ \vtheta - \frac{1}{2\sqrt{nd}}\|\vlambda\|^2 \|\vtheta\|^2.
\end{split}
\end{align}
%
We define the \emph{free energy density} as the expected log-partition function:
%
\begin{align*}
	& \Psi_n^s := \frac{1}{n} \E \left\{ \log \int e^{-H_s(\vlambda) } \tensorl \right\}, \\
	& \Psi_n := \frac{1}{n} \E \left\{ \log \int e^{-H(\vlambda, \vtheta)} \tensorl \tensort \right\}.  
\end{align*}
%
The limit of the free energy density (or equivalently, the mutual information) is of particular interest, as it is related to the Bayesian MMSE through the so-called I-MMSE relation \cite{reeves2016replica}. This limit is also referred to as the \emph{replica-symmetric} (\RS) formulas. The \RS \, formulas for symmetric spiked model and asymmetric spiked model with finite positive aspect ratio has been established in a sequence of papers, for instance, see \cite{miolane2017fundamental,lelarge2019fundamental}. We show that with diverging aspect ratio, the \RS\, formula for model \eqref{model:weak-signal} reduces to that for the symmetric model. 
%

==> introduction_info.tex <==
\section{Introduction}

The problem of low-rank matrix estimation has received enormous attention from extensive body of literatures on random matrix theory, statistical mechanics, statistical inference and computer science. Among the numerous models developed for this purpose, the \emph{spiked model} introduced by Johnstone \cite{johnstone2001distribution} plays a fundamental role, especially for interpreting and understanding high-dimensional asymptotics. This model is also referred to as \emph{deformed ensembles} in the literature of random matrix theory. Theoretical analysis of the spiked models has yielded a number of  important statistical insights, for instance, the prominent BBAP phase transition \cite{baik2005phase,baik2006eigenvalues,johnstone2006high,amini2008high,johnstone2009sparse,ma2013sparse,deshpande2014sparse,deshpande2014information,benaych2011eigenvalues, benaych2012singular,johnstone2020testing,macris2020all}. For the sake of brevity, here we will not attempt to give a complete summary of the historical developments under this category. 

In this paper, we focus on the asymmetric version of the spiked model, also known as the \emph{spiked covariance model}. Like other spiked models, here our observed matrix takes the form of a low-rank signal plus random noise
\begin{align}\label{model:general}
	\bA = s_n \bLambda \bTheta^{\top} + \bZ \in \RR^{n \times d}.
\end{align}
We study the estimation problem under model \eqref{model:general} in the high-dimensional setting where the signal strength is comparable to the noise level. In the above display, we denote by $s_n \in \RR^+$ the signal-to-noise ratio which vanishes as $n$ and $d = d(n)$ go to infinity simultaneously. In order to avoid heavy notations, throughout the paper we will suppress the dependence of $d(n)$ on $n$ and write the single letter $d$ instead. To impose low-rank condition, we assume that the low-rank signal matrix $\bLambda \bTheta$ has rank no larger than $r$ with $r$ a fixed positive integer that does not increase with $n$ and $d$. More precisely, we assume  $\bLambda \in \RR^{n \times r}$ with the $i$-th row denoted by $\Lambda_i \in \RR^r$ and $\bTheta \in \RR^{d \times r}$ with the $j$-th row denoted by $\Theta_j \in \RR^r$. The noise matrix $\bZ \in \RR^{n \times d}$ is assumed to have i.i.d. standard Gaussian entries $(Z_{ij})_{i \leq n, j \leq d} \iidsim \normal(0,1)$, which we further assume is independent of everything else. We comment that although Gaussianity assumption is required throughout the paper, it is possible to eliminate this assumption with more effort due to the prominent universality phenomenon \cite{krzakala2016mutual}. Given one single realization of the observation matrix $\bA$, an important problem that has a wide range of applications is to estimate the low-rank signals $\bLambda$ and $\bTheta$, respectively. The estimation problem described above arises in many machine learning and statistics applications, such as sparse PCA \cite{journee2010generalized,berthet2013optimal,deshpande2014sparse,deshpande2014information}, community detection \cite{abbe2017community,deshpande2017asymptotic}, submatrix localization \cite{kolar2011minimax,hajek2017submatrix} and Gaussian mixture clustering \cite{moitra2010settling,regev2017learning,ndaoud2018sharp,cai2019chime}.

This paper is concerned with the case in which the low-rank signals are structured, and the structural information is known to the estimator before we see the data.  Like in a series of papers \cite{miolane2017fundamental,lelarge2019fundamental,montanari2017estimation,banks2018information}, we model such structural knowledge via taking a Bayesian perspective and assuming the spikes have separable prior distributions that are independent of $n$ and $d$. To be specific, we assume the rows of the low-rank signals obbey $(\Lambda_i)_{i \leq n} \iidsim \mu_{\Lambda}$ and $(\Theta_j)_{j \leq d} \iidsim \mu_{\Theta}$, where $\mu_{\Lambda}$ and $\mu_{\Theta}$ are fixed probability distributions over the $r$-dimensional Euclidean space that are further independent of $(n,d)$. We emphasize that the random matrices $\bLambda, \bTheta$ and $\bZ$ are assumed to be independent of each other. For the sake of simplicity, throughout this paper we assume that $s_n, \mu_{\Lambda}, \mu_{\Theta}$ and $r$ are known to the estimators. From an algorithmic perspective, we comment that empirical Bayes approach is applicable when $s_n, \mu_{\Lambda}, \mu_{\Theta}$ are unknown \cite{zhong2020empirical}. 


The goal of this paper is to compute the Bayesian minimum mean squared error (MMSE) for estimating the low-rank signals $\bLambda$ and $\bTheta$, respectively. As a natural consequence, this allows us to pinpoint the information-theoretic threshold for estimation. More precisely, we can compute the phase transition threshold $s_{c,n}$ such that nontrivial estimation is possible for $s_n > s_{c,n}$, while no algorithm can ourperform random guessing for $s_n < s_{c,n}$. 

Under the proportional asymptotics assumption (i.e., the aspect ratio $d / n$ converges to a finite positive constant as $n$ goes to infinity) and taking $s_n = n^{-1/2}$, \cite{lesieur2015mmse} first establish the limiting expression for Bayesian MMSE under the setting of low-rank matrix estimation. Their derivation is non-rigorous and is based on heuristic tools from statistical mechanics. The conjectured expression is rigorously justified for special instances in \cite{deshpande2014information,deshpande2017asymptotic}. However, their approach highly relies on the fact that approximate message passing (AMP) algorithm achieves Bayes optimality for the specific model considered, thus can not be extended to more general cases. Indeed, their approach fails whenever AMP is sub-optimal. \cite{dia2016mutual} adopt the idea of spatial coupling and prove the so-called  \emph{replica-symmetric} (\RS) formula, which is a fundamental formula lies at the crux of determining the limiting MMSE. Another line of research \cite{lelarge2019fundamental, miolane2017fundamental} proves the \RS\,formula using the Aizenman-Sims-Starr scheme \cite{aizenman2003extended} (also known as cavity computation in the physics literature). More recently, \cite{barbier2019adaptive} presents the adaptive interpolation method which serves as a more unified framework for proving \RS\,formulas. In order to avoid technical intricacies, \cite{el2018estimation} consider free entropy at a fixed overlap and provide a much shorter and more transparent proof of the \RS\,formula comparing to previous approaches. Their proof can be generalized straightforwardly to other models for example spiked tensor with even order. Focusing on phase transition thresholds,  another line of research apply the second moment method and derive upper and lower bounds on the information-theoretic threshold \cite{banks2018information,perry2016optimality,perry2020statistical}. However, in general method of this type is inexact and often a multiplicative gap exists. From an algorithmic perspective, the AMP algorithm, which is a polynomial-time algorithm that can be efficiently implemented, is shown to achieve MMSE for a large region of parameters. One appealing fact about the AMP algorithm is that its asymptotic behavior can be sharply characterized by the \emph{state evolution} quantities, which are simple enough and defined via a sequence of single-letter equations \cite{bayati2011dynamics,montanari2017estimation}. 

As we have mentioned, in all previous attempts, exact derivation of the limiting MMSE requires finite but positive aspect ratio. Past works that are valid for vanishing or diverging aspect ratio usually formulate their results by providing upper and lower bounds for the quantity of interest. These results typically follow with finite-sample guarantee. However, their characterization is usually not sharp, with the existence of a constant or logarithmic multiplicative gap. We refer to \cite{giraud2018partial,ndaoud2018sharp,berthet2013computational,cai2017computational} for exemplar works of this type.

%We consider different regimes in terms of the scales of $s_n$, and provide the corresponding results. As a natural corollary, we derive the exact phase transition threshold of estimation in terms of signal strength. We show that outperforming random guessing is possible above the threshold and impossible below. To present a specific example, we apply our theories to the problem of high-dimensional Gaussian mixture clustering.

\subsection{Our contributions}

Our current work is dedicated to deriving an exact expression of the limiting MMSE for model \eqref{model:general}  under the diverging aspect ratio condition $d / n \to \infty$. We comment that our results can be straightforwardly extended to the vanishing aspect ratio setting via simply exchanging the roles of $n$ and $d$. In this paper, we present the following contributions:
%
\vspace{-0.3cm}
\subsubsection*{Two regimes}
%
\vspace{-0.15cm}
We reveal two regimes, namely, the \emph{strong signal regime} and the \emph{weak signal regime} determined by the scaling of the signal-to-noise ratio $s_n$. In the strong signal regime where $s_n \propto n^{-1/2}$, we show that $\bLambda$ can be estimated consistently up to a rotation. On the other hand, for the estimation of $\bTheta$, we derive expression for the exact limiting MMSE. Our results imply that consistent estimation for $\bTheta$ is in general not attainable under the current setting. In the weak signal regime where $s_n \propto (nd)^{-1/4}$, we prove that no estimator outperforms a naive estimator in terms of estimating $\bTheta$. As for the estimation of $\bLambda$, our main theorems imply the equivalence between model \eqref{model:general} and a symmetric spiked model, the MMSE for the later is established in a series of papers \cite{dia2016mutual,lelarge2019fundamental,barbier2019adaptive,el2018estimation}. In summary, our results unveil asymmetry phenomena between the estimation of $\bLambda$ and $\bTheta$. 
\vspace{-0.3cm}
\subsubsection*{Replica-symmetric formula}
\vspace{-0.15cm}

We establish the replica-symmetric formula in the weak signal regime, which characterizes the limit of the normalized mutual information between the low-rank signal and the observation matrix. In statistical mechanics, RS formula is also related to the convergence of the free energy density. RS formula typically suggests interesting phase transition thresholds. It is also directly associated to the computation of limiting MMSE via the so-called I-MMSE relation. 

%  Our results unveil the asymmetric phenomenon between the estimation of $\bLambda$ and $\bTheta$. To be specific,  As for the estimation of $\bTheta$, we derive the exact limiting MMSE, which implies that consistency is in general not attainable. In the weak signal regime, we prove that no estimator outperforms a naive guessing for the estimation of $\bTheta$. In terms of $\bLambda$, our main theorems establish the equivalence between model \eqref{model:general} and a symmetric spiked model. The MMSE for the later is depicted in \cite{lelarge2019fundamental}. As an application, we apply our theorems to the problem of high-dimensional Gaussian mixture clustering and derive the phase transition thresholds.

 \vspace{0.1cm}

The rest of the paper is organized as follows. \yw{todo}

 
%This allows us to pinpoint the information-theoretic thresholds for estimation in certain parameter regimes. In our setting, this translates into identifying the critical value $C_0^{\ast}$, such that when the "signal strength" (this concept will be discussed in more details later) is no larger than $C_0^{\ast}$, no algorithm can outperform a naive guessing in terms of mean squared error, whereas such algorithm exists when the signal strength is larger than $C_0^{\ast}$, despite the potential computational complexity.
\begin{figure}[h]
\centering
\includegraphics[width=17cm]{figure/low_rank_mat_model.pdf}
\caption{An illustration of the asymmetric spiked model with $d$ much larger than $n$.}
\label{fig:model}
\end{figure}  
\subsection{Notations and conventions}\label{sec:notation}
In this section, we present an incomplete summary of the notations and conventions that will be applied throughout the rest of the paper.

 
For $k \in \NN_+$, we define the set $[k] := \{1,2,\cdots, k\}$. For two sequences of random vectors $\{\bX_{n}\}_{n \in \NN_+} \subseteq \RR^k$ and $\{\bY_{n}\}_{n \in \NN_+}  \subseteq \RR^k$, we say $\bX_{n} \overset{P}{\simeq} \bY_{n}$ if and only if $\|\bX_{n} - \bY_{n}\| = o_p(1)$. Unless stated otherwise, throughout the paper we refer to $\|\cdot\|$ as the Euclidean norm. For vector sequence $\{a_n\}_{n \in \NN_+} \subseteq \RR^k$, we say $a_n = o_n(1)$ if and only if $\|a_n\| \rightarrow 0$ as $n \rightarrow \infty$. For $\{c_n\}_{n \in \NN_+}, \{d_n\}_{n \in \NN_+} \subseteq \RR^+$, we say $c_n \gg d_n$ if and only if $c_n / d_n \rightarrow \infty$. For $n,k \in \NN_+$ and matrix $\bX \in \RR^{n \times k}$ with the $i$-th row denoted by $\bx_i \in \RR^k$, we let $\hat{p}_{\bX}$ be the probability distribution over $\RR^k$, such that for all $\bv \in \RR^k$
\begin{align*}
	\hat{p}_{\bX}(\bv)=\hat{p}_{\bX}(\{\bz: \bz \leq \bv\}) := \frac{1}{n}\sum_{i = 1}^n\mathbbm{1}\{ \bx_i \leq \bv \}.
\end{align*}
In the above display, $\leq$ stands for element-wise comparison between vectors, i.e., $\mathbbm{1}\{\bx \leq \bv\} = 1$ if and only if $x_i \leq v_i$ for all $i \in [k]$.  

%For matrix $\bM$, we denote the $k$-th largest singular value of $\bM$ by $\sigma_k(\bM)$. Furthermore, we let $\|\bM\|_{\rm{op}} := \sigma_1(\bM)$, $\|\bM\|_F$ be the Frobenius norm of $\bM$, and $\Tr(\bM)$ be the trace of $\bM$. 

For $k \in \NN_+$, we denote by $S_k^+$ the set of positive semi-definite matrices in $\RR^{k \times k}$, and denote by $\mathcal{O}(k)$ the set of orthogonal matrices in $\RR^{k \times k}$. For $\bM \in S_k^+$, we let $\bM^{1/2} \in S_k^+$ be any positive semi-definite matrix such that $\bM = \bM^{1/2}\bM^{1/2}$. For $k, n \in \NN_+$ and $\bX,\bY \in \RR^{n \times k}$, we define $[ \bX, \bY ] := \bX^{\top}\bY \in \RR^{k \times k}$. For $\bW \in \RR^{n \times k}$ and $1 \leq a < b \leq n$, $1 \leq c < d \leq k$, $a,b,c,d \in \NN_+$, we let $\bW_{a:b,c:d} \in \RR^{(b - a + 1) \times (d - c + 1)}$ be the submatrix of $\bW$ which is the slice corresponding to its $a$-th to $b$-th rows and $c$-th to $d$-th columns. We let $\bW = \bU \bSigma \bV^{\top}$ be the singular value decomposition of $\bW$ such that $\bSigma$ is a diagonal matrix with descending diagonal entries, the columns of $\bU$ are the left singular vectors of $\bW$ and the columns of $\bV$ are the right singular values of $\bW$. For $m \in \NN_+$, we let  $\SVD_m(\bW) = \bU_{1:m} \bSigma_{1:m,1:m} \bV_{1:m}^{\top}$,  where $\bU_{1:m} = \bU_{1:n,1:m} \in \RR^{n \times m}$ and $\bV_{1:m} = \bV_{1:n,1:m}\in \RR^{k \times m}$. Notice that the choice of $\SVD_m(\bW)$ might not be unique. In this case, we randomly pick one among all eligible matrices. 
  
 With a slight abuse of notations, in this paper we will use the capital letter $C$ to represent various numerical constants. Unless stated otherwise, we use capital bold letters $\bLambda, \bTheta$ to represent the low-rank signals that appear in model definition \eqref{model:general} with the $i$-th rows of which being $\Lambda_i$ and $\Theta_i$, respectively. We use non-bold letters $\Lambda$ and $\Theta$ to represent length $r$ random vectors drawn from probability distributions $\mu_{\Lambda}$ and $\mu_{\Theta}$. We sometimes need to express the posterior distribution of $(\bLambda, \bTheta)$ given particular observations. In this case, we use the lower case letters $\vtheta, \vlambda, \lambda_i, \theta_i$ to represent variables corresponding to $(\bTheta, \bLambda, \Lambda_i, \Theta_i)$ in the posterior distribution. More precisely, here we have $\vlambda \in \RR^{n \times r}$, $\vtheta \in \RR^{d \times r}$ and  $\lambda_i, \theta_i \in \RR^r$.
 
 
% Since we work with Bayesian models, we will need to represent the posterior distribution of $(\bLambda, \bTheta)$ in later parts of the paper. We use lower case letters $\vtheta, \vlambda, \lambda_i, \theta_i$ to represent the variables corresponding to $(\bTheta, \bLambda, \Lambda_i, \Theta_i)$ in the posterior distribution given $\bA$. Here, $\vlambda \in \RR^{n \times r}$, $\vtheta \in \RR^{d \times r}$ and  $\lambda_i, \theta_i \in \RR^r$. 
 
 
  
 
 




==> lower-bound.tex <==
\section{Information-theoretic lower bound}

In this section, we consider the information-theoretic lower bound of estimating $\blambda$. We consider the minimum mean squared error defined as follows(this metric is able to break the symmetry when $\Lambda$ is symmetrically distributed). 
\begin{align}\label{eq:MMSEA}
 \MMSE_n(\bA) = \min\limits_{\hat{M}(\bA)} \frac{1}{n^2} \E\left[ \left\| \bLambda\bLambda^\intercal - \hat{M}(\bA) \right\|_{F}^2 \right],
\end{align}
where $\hat{M}(\bA)$ is any measurable function of the observations $\bA$. For the sake of completeness, here we reproduce the definition of the following function proposed in \cite{lelarge2019fundamental}:
\begin{align*}
	& F_n(s) = \frac{1}{n} \E\left[ \log \left( \int \exp\left( \sum\limits_{i < j }\sqrt{s}\lambda_i\lambda_j W_{ij} + \frac{s}{n}\Lambda_i\Lambda_j \lambda_i\lambda_j - \frac{s}{2n} \lambda_i^2\lambda_j^2 \right)\tensorl \right)  \right],\\
	& \cF: (s, q) \in \RR_+^2  \mapsto - \frac{s}{4}q^2 + \E\log \left(\int \exp\left( \sqrt{sq}Z\lambda + sq\lambda \Lambda - \frac{s}{2}q\lambda^2 \right)\dd P_{\Lambda}(\lambda) \right),
\end{align*}
For the purpose of comparison, we introduce the symmetric model and its corresponding minimum mean squared error:
\begin{align}
	& \bY = \frac{q_{\Theta}^2}{n} \bLambda \bLambda^\intercal + \bW, \qquad \bW \sim \frac{1}{\sqrt{n}} \GOE(n), \label{model:symmetric} \\
	& \MMSE_n(\bY) = \min\limits_{\hat{M}(\bY)} \frac{1}{n^2} \E\left[ \left\| \bLambda\bLambda^\intercal - \hat{M}(\bY) \right\|_{F}^2 \right]. \label{eq:MMSEY}
\end{align}
%
Then we have the following theorem regarding the minimum mean squared error:
\begin{theorem}\label{thm:lower-bound}
	Assume $\E[\Theta] = \E[\Theta^3] = 0$, $\Theta, \Lambda$ are sub-gaussian random variables, and $d / n \rightarrow \infty$, then for all but countably many values of $q_{\Theta}^2$, we have
	\begin{align*}
		\liminf\limits_{n,d \rightarrow \infty}\MMSE_n(\bA) \geq \E[\Lambda^2]^2 - q^{\ast}(q_{\Theta}^2)^2.
	\end{align*}
	Furthermore, the equality holds when (1) $d / n^3 \rightarrow \infty$, (2) AMP achieves optimal MMSE under the symmetric spiked model, in this case AMP also achieves optimal MMSE under our proposed model(\yw{to be stated formally}).
\end{theorem}


==> weak-signal.tex <==
\section{Weak signal regime}\label{sec:weak-signal}
In this section, we consider the weak signal regime where $s_n = 1 / \sqrt[4]{nd}$. The model of interest can be expressed as
%
\begin{align}\label{model:weak-signal}
	\bA = \frac{1}{\sqrt[4]{nd}}\blambda \btheta^\intercal + \bZ \in \mathbb{R}^{n \times d}\, .
\end{align}
% 
For the simplicity of notations we define $r_n := \sqrt[4]{d / n}$. Under our infinite aspect ratio assumption we see that $r_n \to \infty$ as $n,d \to \infty$. 
 
\subsection{Estimation of  $\bTheta$}\label{sec:weak-regime-theta}

We first consider the estimation of $\bTheta$ in the weak signal regime. We claim that in this case no estimator outperforms a naive one in terms of asymptotic mean squared error. Indeed, we show that the mean squared error achieved by simply taking the prior mean agrees asymptotically with the Bayesian MMSE with extra information. 
 
\begin{theorem}\label{thm:weak-signal-theta}
Under Assumption \ref{assumption:second-moment} and model \eqref{model:weak-signal}, we let $n, d \rightarrow \infty$ simultaneously with $d / n \rightarrow \infty$. Then for any $\bhtheta \in \mathbb{R}^{d \times r}$ being an estimator of $\btheta$ based on observation $\bA$, we have 
	\begin{align*}
		 \liminf\limits_{n,d \rightarrow \infty}\frac{1}{d} \E[ \|\bhtheta - \btheta\|_F^2] \geq rq_{\Theta} - \|\E_{\Theta \sim \mu_{\Theta}}[\Theta]\|^2. 
	\end{align*}
	If we further assume $\mu_{\Theta}$ has bounded fourth moment, then for any $\hat\bM \in \RR^{d \times d}$ being an estimator of $\bTheta \bTheta^{\top}$ using observation $\bA$
	\begin{align*}
		 \liminf\limits_{n,d \rightarrow \infty}\frac{1}{d^2} \E[ \|\bTheta \bTheta^{\top} - \hat\bM\|_F^2 ] \geq rq_{\Theta}^2 - \|\E_{\Theta \sim \mu_{\Theta}}[\Theta]\|^4_2.
	\end{align*}
	Notice that the above lower bounds are achieved by the naive estimators $\bhtheta = \E[\bTheta] \in \RR^{d \times r}$ and $\hat\bM = \E[\bTheta \bTheta^{\top}] \in \RR^{d \times d}$. 
\end{theorem}
%
In order to prove \cref{thm:weak-signal-theta}, we follow similar idea of \cref{thm:strong-signal-theta-lower-bound} and reveal extra information $\bLambda$. We then show that the posterior distribution of $\bTheta$ conditioning on $(\bA, \bLambda)$ can be factored in a desired manner that is similar to \cref{eq:5}, thus allows the exact derivation of MMSE. Finally, we prove that this MMSE agrees asymptotically with the mean squared error achieved by a naive estimator. We leave the details of the proof to Appendix \ref{proof:thm:weak-signal-theta}. 


\subsection{Estimation of  $\bLambda$}\label{sec:weak-regime-estimate-lambda}
%
In this section, we focus on the estimation of $\blambda$ under the weak signal regime. Due to technical reasons, for this part we  consider only the matrix mean squared error. More precisely, our goal is to provide asymptotic characterization of the matrix MMSE
\begin{align}\label{eq:MMSEA}
 \MMSE_n(\bA) := \min\limits_{\hat{M}(\bA)} \frac{1}{n^2} \E\left[ \left\| \bLambda\bLambda^\intercal - \hat{M}(\bA) \right\|_{F}^2 \right],
\end{align} 
%
where $\hat{M}(\bA) \in \RR^{n \times n}$ is any estimator of $\bLambda \bLambda^{\top}$ constructed based on observation matrix $\bA$. In the rank-one case $r = 1$, if $\E_{\Theta \sim \mu_{\Theta}}[\Theta] \neq 0$, then direct computation reveals  that the naive estimator $r_n^{-1}\bA\by$ with $\by = \frac{1}{\sqrt{d}}\E[\Theta]^{-1}\vec{1}_d$ is consistent for $\blambda$ in terms of vector mean squared error:
%
\begin{align*}
	\frac{1}{n}\left\| r_n^{-1} \bA \by - \bLambda \right\|_2^2 \toP 0. 
\end{align*} 
%
In this case, consistent estimation evaluated in matrix mean squared error naturally follows, suggesting $\Theta$ with non-vanishing expectation significantly reduces the difficulty of estimation. In the multi-dimensional setting, non-zero mean vector leads to consistent estimation of $\bLambda$ projected onto the direction determined by the mean vector $\E_{\Theta \sim \mu_{\Theta}}[\Theta]$. For the remainder of this section, we focus on the more challenging regime which assumes $\E_{\Theta \sim \mu_{\Theta}}[\Theta] = \mathbf{0}_r$. In addition, we require $\mu_{\Theta}$ has zero third order moment. 
%
\begin{assumption}\label{assumption:info}
	We assume $\E_{\Theta \sim \mu_{\Theta}}[\Theta] =  \mathbf{0}_r$, $\E_{\Theta \sim \mu_{\Theta}}[\Theta  \otimes \Theta \otimes \Theta] = \bold{0}_{r \times r \times r}$ where $\otimes$ denotes the tensor product. Furthermore, we require that $\mu_{\Theta}, \mu_{\Lambda}$ are sub-Gaussian distributions over the $r$-dimensional Eulidean space.\footnote{For a formal definition of sub-Gaussian random vectors, see \cite{vershynin2018high}.} 
\end{assumption}
%
Our main theorem roughly says that in terms of estimating $\bLambda \bLambda^{\top}$, the asymmetric model \eqref{model:weak-signal} of interest is equivalent to a symmetric spiked model  under the proposed regularity conditions. Under the symmetric model, the observation takes the form of an $n \times n$ symmetric matrix $\bY$, which is detailed as follows:
%
\begin{align}
	\bY = \frac{q_{\Theta}}{n} \bLambda  \bLambda^\intercal + \bW, \qquad \bW \sim \frac{1}{\sqrt{n}} \GOE(n). \label{model:symmetric}
\end{align}
%
In the above display, $\bLambda \in \RR^{n \times r}$ is the same as the low-rank signal defined in the asymmetric model, and we require the noise matrix $\bW$ is independent of $\bLambda$. Similarly, we define the Bayesian MMSE for model \eqref{model:symmetric} as
%
\begin{align}
	\MMSE_n(\bY) := \min\limits_{\hat{M}(\bY)} \frac{1}{n^2} \E\left[ \left\| \bLambda\bLambda^\intercal - \hat{M}(\bY) \right\|_{F}^2 \right]. \label{eq:MMSEY}
\end{align}
%
Note that the Bayesian MMSE is achieved by the posterior mean. In order to analyze MMSE defined in \cref{eq:MMSEA} and \cref{eq:MMSEY}, we first study the posterior distributions which can be written as
%
\begin{align*}
	& \dd\P(\bLambda = \vlambda \mid \bY) = \frac{e^{-H_s(\vlambda)} \tensorl}{\int e^{-H_s(\vlambda)} \tensorl }, \\
	& \dd\P(\bLambda = \vlambda, \bTheta = \vtheta \mid \bA) = \frac{e^{-H(\vlambda, \vtheta)} \tensort\tensorl}{\int e^{-H(\vlambda, \vtheta)} \tensort\tensorl},
\end{align*} 
where $ \tensorl$ ($\tensort$) is the product distribution over $\RR^n$ ($\RR^d$) with each coordinate having marginal distribution $\mu_{\Lambda}$ ($\mu_{\Theta}$), and $H_s, H$ are the (random) Hamiltonians for model \eqref{model:symmetric} and \eqref{model:weak-signal}, respectively
%
\begin{align}\label{eq:Hs-and-H}
\begin{split}
	& H_s(\vlambda ) := \, \frac{q_{\Theta}^2}{2n}\langle \bLambda, \vlambda \rangle^2 + \frac{q_{\Theta}}{2}\vlambda^\intercal\bW \vlambda - \frac{q_{\Theta}^2}{4n}\|\vlambda\|_2^4, \\
	& H(\vlambda, \vtheta) := \frac{1}{\sqrt{nd}}\langle \bLambda, \vlambda \rangle \langle \bTheta, \vtheta \rangle + \frac{1}{\sqrt[4]{nd}}  \vlambda^{\top}\bZ \vtheta - \frac{1}{2\sqrt{nd}}\|\vlambda\|_2^2 \|\vtheta\|_2^2.
\end{split}
\end{align}
%
Following the terminology of statistical mechanics, the \emph{free energy densities} are defined as the expected log-partition functions (also known as log normalizing constant):
%
\begin{align*}
	& \Psi_n^s := \frac{1}{n} \E \log \int e^{-H_s(\vlambda) } \tensorl, \\
	& \Psi_n := \frac{1}{n} \E \log \int e^{-H(\vlambda, \vtheta)} \tensorl \tensort.  
\end{align*}
%
The limit of the free energy density (or equivalently, the mutual information) is of particular interest, as it is related to the Bayesian MMSE through the so-called I-MMSE relation \cite{reeves2016replica}. The limit of the above quantities are also referred to as the \emph{replica-symmetric} (\RS) formulas. The \RS \, formulas for symmetric spiked model and asymmetric spiked model with finite positive aspect ratio has been established in a sequence of papers, for instance, see \cite{miolane2017fundamental,lelarge2019fundamental}. Here, we prove that in the diverging aspect ratio regime with $d / n \to \infty$, the \RS\, formula for the asymmetric spiked model \eqref{model:weak-signal} reduces to that for the symmetric model. 
%
\begin{theorem}\label{thm:free-energy}
	Under Assumption \ref{assumption:second-moment},  \ref{assumption:info} and model \eqref{model:weak-signal}, we let $n,d \rightarrow \infty$ simultaneously with $d / n \rightarrow \infty$. Then as $n,d \to \infty$ we have
	\begin{align*}
		\lim_{n \to \infty} \Psi_n^s = \lim_{n,d \to \infty} \Psi_n = \sup_{\bQ \in S_r^+} \cF(q_{\Theta}^2, \bQ),
	\end{align*}
	where the second equality is by Theorem 42 in \cite{lelarge2019fundamental}. 
\end{theorem} 
%
Leveraging Gaussian integration by parts, we see that the partial derivative $\frac{\partial}{\partial q_{\Theta}} \Psi_n^s$ is directly related to $\MMSE_n(\bY)$, while the relationship between $\frac{\partial}{\partial q_{\Theta}} \Psi_n$ and $\MMSE_n(\bA)$ is unclear. In order to compute $\MMSE_n(\bA)$, we add to both models a small perturbation
%
\begin{align*}
	\bY'(\ep) := \frac{\sqrt{n}}{n} \bLambda \bLambda^{\top} + \bW', 
\end{align*}
%
where $\ep > 0$, $\bW' \overset{d}{=} \frac{1}{\sqrt{n}} \GOE(n)$ and $\bW' \perp \bLambda$. In words, our theorem proceeds by showing that the free energy densities of these two models with extra perturbation still agree asymptotically. Then we take the partial derivatives of the free energy densities with respect to $\ep$. In this way, we manage to retrieve information about the connection between $\MMSE_n(\bA)$ and $\MMSE_n(\bY)$ through the I-MMSE relation. A direct implication of this procedure is that  $\MMSE_n(\bA)$ is asymptotically no larger than $\MMSE_n(\bY)$. The later quantity is further given explicitly by \cref{prop:symmetric-spike}. 

\begin{theorem}\label{thm:lower-bound}
	Under Assumption \ref{assumption:second-moment}, \ref{assumption:info} and model \eqref{model:weak-signal}, we let $n,d \rightarrow \infty$ simultaneously with $d / n \rightarrow \infty$, then for all but countably many values of $q_{\Theta}$, we have
	\begin{align}\label{eq:thm-lower-bound}
		\liminf\limits_{n,d \rightarrow \infty}\MMSE_n(\bA) \geq \lim\limits_{n \rightarrow \infty} \MMSE_n(\bY). 
	\end{align}
\end{theorem}
%
The proofs of \cref{thm:free-energy} and \cref{thm:lower-bound} are outlined in \cref{sec:proof-of-thm-lower-bound-lower-bound} and \cref{sec:proof-of-thm:lower-bound} in the appendix respectively for distributions with bounded support, and relaxed to more general distributions in \cref{section:reduction-to-bdd-support}. The symmetric model \eqref{model:symmetric} can be solved via the AMP algorithm. For many choices of parameters $(q_{\Theta}, \mu_{\Lambda})$, AMP with appropriate non-linearites asymptotically achieves  Bayesian MMSE. Due to space limit, in this paper we will not cover a detailed discussion of when AMP achieves Bayes optimality. We refer the interested readers to \cite[Section 2.4]{montanari2017estimation} for more details. 
 
% Informally speaking, in our second main theorem, we show that the inequality \eqref{eq:thm-lower-bound} in \cref{thm:lower-bound} can be replaced by an equality with limit inferior replaced by limit if additionally, at least one of the following conditions hold: (a) $d$ grows much faster than $n$; (b) $d$ grows faster than $n$, but not too fast; (c) AMP asymptotically achieves Bayesian MMSE for model \ref{model:symmetric}. To be formal, we state the following theorem:
%
\begin{theorem}\label{thm:upper-bound}
	Under the conditions of Theorem \ref{thm:lower-bound}, if in addition, we assume at least one of the following conditions holds:
	\begin{enumerate}
		\item[(a)] $d n^{-3}(\log n)^{-6} \rightarrow \infty$,
		\item[(b)] $n^{6/5}(\log d)^{-8/5} \gg d \gg n$ and $\mu_{\Lambda}$ has bounded support, 
		%\item[(c)] Under the symmetric model \eqref{model:symmetric}, AMP algorithm with spectral initialization  asymptotically achieves the Bayesian MMSE defined in \cref{eq:MMSEY},
		\item[(c)] Condition \ref{condition:stationary} holds for $s = q_{\Theta}^2$,
	\end{enumerate}
	then for all but countably many values of  $q_{\Theta}$, we have $\lim_{n,d \rightarrow \infty} \MMSE_n(\bA) = \lim_{n \rightarrow \infty} \MMSE_n(\bY)$. 
\end{theorem}
%
We defer the proof of \cref{thm:upper-bound} to \cref{sec:proof-thm:upper-bound} in the appendix. Results presented in \cref{sec:weak-regime-theta} and \cref{sec:weak-regime-estimate-lambda} imply that in the weak signal regime it is possible to partially recover $\bLambda$ while impossible to recover $\bTheta$ better than a naive estimator. We illustrate in \cref{sec:real-data} the existence of such asymmetric phenomenon in real world datasets. 

\yw{I only proved the theorem with r = 1, shall I do the proof for $r \geq 2$?}

 







